Time-Uniform Self-Normalized Concentration for Vector-Valued Processes

Self-normalized processes arise naturally in many learning-related tasks. While self-normalized concentration has been extensively studied for scalar-valued processes, there are few results for multidimensional processes outside of the sub-Gaussian setting. In this work, we construct a general, self-normalized inequality for multivariate processes that satisfy a simple yet broad sub-$\psi$ tail condition, which generalizes assumptions based on cumulant generating functions. From this general inequality, we derive an upper law of the iterated logarithm for sub-$\psi$ vector-valued processes, which is tight up to small constants. We show how our inequality can be leveraged to derive a variety of novel, self-normalized concentration inequalities under both light and heavy-tailed observations. Further, we provide applications in prototypical statistical tasks, such as parameter estimation in online linear regression, autoregressive modeling, and bounded mean estimation via a new (multivariate) empirical Bernstein concentration inequality.

==> images/CGF_compare.tex <==
\begin{tikzpicture}[%
  >=Stealth,              % arrow tips
  node distance=2.5cm,
  every node/.style={font=\sffamily},
  box/.style={%
    draw,
    rounded corners,
    minimum width=2.5cm,
    minimum height=1.2cm,
    align=center
  }
]

%--- Nodes ---
\node[box] (gaus)  {Sub-Gaussian};
\node[box] (pois) [below=2cm of gaus]  {Sub-Poisson};
\node[box] (exp)  [right=3cm of pois]   {Sub-exponential};
\node[box] (gam)  [above=2cm of exp]  {Sub-gamma};

%--- Edges ---

% 1) Sub-Bernoulli <--> Sub-Gaussian
\draw[->] (gaus) -- (pois);
\draw[->] (pois) -- (exp);
\draw[->] (exp) -- (gam);

\end{tikzpicture}
